Neuroevolution-based Classifiers for Deforestation Detection in Tropical Forests

Tropical forests represent the home of many species on the planet for flora and fauna, retaining billions of tons of carbon footprint, promoting clouds and rain formation, implying a crucial role in the global ecosystem, besides representing the home to countless indigenous peoples. Unfortunately, millions of hectares of tropical forests are lost every year due to deforestation or degradation. To mitigate that fact, monitoring and deforestation detection programs are in use, in addition to public policies for the prevention and punishment of criminals. These monitoring/detection programs generally use remote sensing images, image processing techniques, machine learning methods, and expert photointerpretation to analyze, identify and quantify possible changes in forest cover. Several projects have proposed different computational approaches, tools, and models to efficiently identify recent deforestation areas, improving deforestation monitoring programs in tropical forests. In this sense, this paper proposes the use of pattern classifiers based on neuroevolution technique (NEAT) in tropical forest deforestation detection tasks. Furthermore, a novel framework called e-NEAT has been created and achieved classification results above $90\%$ for balanced accuracy measure in the target application using an extremely reduced and limited training set for learning the classification models. These results represent a relative gain of $6.2\%$ over the best baseline ensemble method compared in this paper

==> results/allMethods.tex <==
%\begin{tabular}{lrrrr}
%\toprule
%  &  \multicolumn{4}{c}{Balanced accuracy} \\
%Method &   Mean &  Std &    Min &    Max \\
%\midrule
%e-NEAT                   &    0.869 &  0.053 &  0.777 &  0.904    \\
%e-NEAT\_mode             &    \textbf{0.900} &  0.010 &  0.886 &  0.910    \\
%e-NEAT\_topAnns          &    0.856 &  0.051 &  0.777 &  0.911    \\
%e-NEAT\_errorCorrelation &    0.850 &  0.109 &  0.656 &  0.910    \\
%e-NEAT\_topDiversity     &    0.848 &  0.069 &  0.748 &  0.915    \\
%AdaBoost                 &    0.472 &  0.000 &  0.472 &  0.472    \\
%Random Forest            &    0.822 &  0.031 &  0.781 &  0.861    \\
%Bagging Classifier       &    0.841 &  0.037 &  0.795 &  0.878    \\
%Extra Trees              &    0.824 &  0.024 &  0.793 &  0.859    \\
%Gradient Boosting        &    0.798 &  0.009 &  0.785 &  0.809    \\ \hline
%MLP Classifier           &    0.867 &  0.009 &  0.857 &  0.882    \\
%KNN                      &    0.796 &  0.000 &  0.796 &  0.796    \\
%Gaussian NB              &    0.831 &  0.000 &  0.831 &  0.831    \\
%Decision Tree            &    0.719 &  0.069 &  0.635 &  0.770    \\
%SVM Linear               &    0.887 &  0.000 &  0.887 &  0.887    \\
%SVM Poly                 &    0.755 &  0.000 &  0.755 &  0.755    \\
%SVM Rbf                  &    0.819 &  0.000 &  0.819 &  0.819    \\
%\bottomrule
%\end{tabular}

%\begin{table}[ht!]
%\centering
\resizebox{9cm}{!}{
\begin{tabular}{llrrrr}
\toprule
 & &  \multicolumn{4}{c}{\textbf{Balanced Accuracy}} \\
& \textbf{Method} &   \textbf{Average} &  \textbf{Std} &    \textbf{Min.} &    \textbf{Max.} \\
\toprule
\multirow{ 7}{*}{\textbf{Single}} & MLP Classifier           &    86.7 &  9.0 &  85.7 &  88.2    \\
&KNN                      &    79.6 &  0.0 &  79.6 &  79.6    \\
&Gaussian NB              &    83.1 &  0.0 &  83.1 &  83.1    \\
&Decision Tree            &    71.9 &  6.9 &  63.5 &  77.0    \\
&SVM Linear               &    88.7 &  0.0 &  88.7 &  88.7    \\
&SVM Poly                 &    75.5 &  0.0 &  75.5 &  75.5    \\
&SVM Rbf                  &    81.9 &  0.0 &  81.9 &  81.9    \\

\midrule
\multirow{10}{*}{\textbf{Ensemble}} &AdaBoost                 &    47.2 &  0.0 &  47.2 &  47.2    \\
&Random Forest            &    82.2 &  3.1 &  78.1 &  86.1    \\
&Bagging Classifier       &    84.1 &  3.7 &  79.5 &  87.8    \\
&Extra Trees              &    82.4 &  2.4 &  79.3 &  85.9    \\
&Gradient Boosting        &    79.8 &  9.0 &  78.5 &  80.9    \\ %\cline{2-3} 
&e-NEAT                   &    86.9 &  5.3 &  77.7 &  90.4    \\
& \textbf{e-NEAT\_mode}              &    \textbf{90.0} &  1.0 &  \textbf{88.6} &  \textbf{91.0}    \\
&e-NEAT\_topAnns          &    85.6 &  5.1 &  77.7 &  91.1    \\
&e-NEAT\_errorCorrelation  &    85.0 &  10.9 &  65.6 &  91.0    \\
&e-NEAT\_topDiversity     &    84.8 &  6.9 &  74.8 &  91.5    \\
\bottomrule
\end{tabular}
}
%\end{table}

\begin{table}[ht!]
\resizebox{9cm}{!}{
\begin{tabular}{lrrrr}
\toprule
 & &  \multicolumn{4}{c}{\textbf{Balanced Accuracy}} \\
& \textbf{Method} &   \textbf{Average} &  \textbf{Std} &    \textbf{Min.} &    \textbf{Max.} \\
\toprule
AdaBoost                 &    47.2 &  0.0 &  47.2 &  47.2    \\
Random Forest            &    82.2 &  3.1 &  78.1 &  86.1    \\
Bagging Classifier       &    84.1 &  3.7 &  79.5 &  87.8    \\
Extra Trees              &    82.4 &  2.4 &  79.3 &  85.9    \\
Gradient Boosting        &    79.8 &  9.0 &  78.5 &  80.9    \\ %\cline{2-3} 
e-NEAT                   &    86.9 &  5.3 &  77.7 &  90.4    \\
 \textbf{e-NEAT\_mode}              &    \textbf{90.0} &  1.0 &  \textbf{88.6} &  \textbf{91.0}    \\
e-NEAT\_topAnns          &    85.6 &  5.1 &  77.7 &  91.1    \\
e-NEAT\_errorCorrelation  &    85.0 &  10.9 &  65.6 &  91.0    \\
e-NEAT\_topDiversity     &    84.8 &  6.9 &  74.8 &  91.5    \\
\bottomrule
\end{tabular}
}
\end{table}

